OpenFlamingo: An Open-Source Framework for Training Large Autoregressive Vision-Language Models

We introduce OpenFlamingo, a family of autoregressive vision-language models ranging from 3B to 9B parameters. OpenFlamingo is an ongoing effort to produce an open-source replication of DeepMind's Flamingo models. On seven vision-language datasets, OpenFlamingo models average between 80 - 89% of corresponding Flamingo performance. This technical report describes our models, training data, hyperparameters, and evaluation suite. We share our models and code at https://github.com/mlfoundations/open_flamingo.

==> tables/smalltable_rices.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c||c|c||c|c|c|c|c}
% \textbf{Benchmark} & \textbf{Shots} & \rotatebox{90}{\textbf{\fl-3B} \cite{alayrac2022flamingo}} & \rotatebox{90}{\textbf{\fl-9B} \cite{alayrac2022flamingo}} & \rotatebox{90}{\href{https://huggingface.co/openflamingo/OpenFlamingo-3B-vitl-mpt1b}{\oftb}} & \rotatebox{90}{\parbox{4cm}{\centering \href{https://huggingface.co/openflamingo/OpenFlamingo-3B-vitl-mpt1b-langinstruct}{\oftb} \\ (Instruct)}} & \rotatebox{90}{\href{https://huggingface.co/openflamingo/OpenFlamingo-4B-vitl-rpj3b}{\offb}} & \rotatebox{90}{\parbox{4cm}{\centering \href{https://huggingface.co/openflamingo/OpenFlamingo-4B-vitl-rpj3b-langinstruct}{\offb} \\ (Instruct)}} & \rotatebox{90}{\href{https://huggingface.co/openflamingo/OpenFlamingo-9B-vitl-mpt7b}{\ofnb}}\\ 
\textbf{Benchmark} & \textbf{Shots} & \textbf{Fl-3B} & \textbf{Fl-9B} & \textbf{OF-3B} & \textbf{OF-3B (I)} & \textbf{OF-4B} & \textbf{OF-4B (I)} & \textbf{OF-9B}\\ 
\hline
\multirow{5}{*}{\textbf{\coco} \cite{Chen2015MicrosoftCC}} & 0 & 73.0 & 79.4 & \textbf{81.6} & 79.0 & 75.9 & 79.5 & 76.8 \\
& 4 & 85.0 & \textbf{93.1} & 91.3 & 90.5 & 89.0 & 92.7 & \textbf{93.1} \\
& 32 & 99.0 & 106.3 & 105.5 & 104.1 & 105.1 & 107.8 & \textbf{109.0} \\
\hline
\multirow{5}{*}{\textbf{\flickr} \cite{Young2014FromID}} & 0 & 60.6 & \textbf{61.5} & 46.0 & 45.0 & 36.3 & 43.0 & 39.2 \\
& 4 & 72.0 & \textbf{72.6} & 54.0 & 53.9 & 48.9 & 53.6 & 52.2 \\
& 32 & 71.2 & \textbf{72.8} & 65.5 & 64.6 & 56.2 & 56.6 & 63.0 \\
\hline
\multirow{5}{*}{\textbf{\vqav} \cite{Agrawal2015VQAVQ}} & 0 & 49.2 & 51.8 & 44.5 & 44.0 & 45.3 (old) & 46.6 & \textbf{53.0} \\
& 4 & 53.2 & \textbf{56.3} & 45.9 & 45.3 & 49.7 (old) & 49.6 & 55.1 \\
& 32 & 57.1 & \textbf{60.4} & 49.1 & 46.7 & 39.4 (old) & 48.9 & 56.8 \\
\hline
\multirow{5}{*}{\textbf{\okvqa} \cite{Marino2019OKVQAAV}} & 0 & 41.2 & \textbf{44.7} & 28.6 & 29.2 & 31.0 & 32.0 & 38.3 \\
& 4 & 43.3 & \textbf{49.3} & 31.0 & 31.4 & 34.8 & 35.1 & 42.0 \\
& 32 & 45.9 & \textbf{51.0} & 35.1 & 34.6 & 28.7 & 36.5 & 46.3 \\
\hline
\multirow{5}{*}{\textbf{\textvqa} \cite{Singh2019TowardsVM}} & 0 & 30.1 & \textbf{31.8} & 24.5 & 26.0 & 22.8 & 23.5 & 28.3 \\
& 4 & 32.7 & 33.6 & 27.2 & 28.9 & 26.7 & 28.9 & \textbf{34.2} \\
& 32 & 30.6 & \textbf{32.6} & 29.2 & 29.0 & 17.93 & 23.0 & 31.1 \\
\hline
\multirow{5}{*}{\textbf{\vizwiz} \cite{Gurari2018VizWizGC}} & 0 & 28.9 & 28.8 & 23.8 (old) & 32.6 & 28.0 & 30.1 & \textbf{34.6} \\
& 4 & 34.0 & 34.9 & 33.8 (old) & 39.0 & 37.4 & 36.6 & \textbf{41.0} \\
& 32 & 45.5 & 44.0 & 44.9 (old) & 45.9 & 27.3 & 36.4 & \textbf{46.4} \\
\hline
\multirow{5}{*}{\textbf{\hms} \cite{Kiela2020TheHM}} & 0 & 53.7 & 57.0 & 63.9 & 65.2 & 64.8 & 66.2 & \textbf{67.1}\\
& 4 & 53.6 & 62.7 & 66.1 & 65.7 & 65.4 & 66.8 & \textbf{70.1}\\
& 32 & 56.3 & 63.5 & 68.2 & 67.7 & 64.4 & 62.2 & \textbf{73.6} \\
\hline
\end{tabular}
}
\caption{Evaluation results using RICES across seven vision-language datasets using 0, 4, and 32 in-context examples. \of models are notably weaker than their \fl counterparts on \flickr and \okvqa. ``OF-3B (I)'' refers to \oftb (Instruct), the 3B model trained with a language-instruction-tuned backbone, while ``Fl-3B'' refers to \fl-3B. \fl results taken from \citet{alayrac2022flamingo}. The highest number in each row is bolded. Full results with standard deviations are in Table~\ref{tab:eval_large_rices}.\vspace{0.5em}}
\label{tab:eval_short_rices}
\end{table*}
